Improving Data Efficiency for Plant Cover Prediction with Label Interpolation and Monte-Carlo Cropping

The plant community composition is an essential indicator of environmental changes and is, for this reason, usually analyzed in ecological field studies in terms of the so-called plant cover. The manual acquisition of this kind of data is time-consuming, laborious, and prone to human error. Automated camera systems can collect high-resolution images of the surveyed vegetation plots at a high frequency. In combination with subsequent algorithmic analysis, it is possible to objectively extract information on plant community composition quickly and with little human effort. An automated camera system can easily collect the large amounts of image data necessary to train a Deep Learning system for automatic analysis. However, due to the amount of work required to annotate vegetation images with plant cover data, only few labeled samples are available. As automated camera systems can collect many pictures without labels, we introduce an approach to interpolate the sparse labels in the collected vegetation plot time series down to the intermediate dense and unlabeled images to artificially increase our training dataset to seven times its original size. Moreover, we introduce a new method we call Monte-Carlo Cropping. This approach trains on a collection of cropped parts of the training images to deal with high-resolution images efficiently, implicitly augment the training images, and speed up training. We evaluate both approaches on a plant cover dataset containing images of herbaceous plant communities and find that our methods lead to improvements in the species, community, and segmentation metrics investigated.

==> tables/daily_mc0.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{3}{|c}{0} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{0} \\
{} &                      MSAE &                       IoU &                       DPC \\
\textbf{Epochs} &                           &                           &                           \\
\midrule
\textbf{3     } &  \makecell{0.494\\±0.003} &  \makecell{0.205\\±0.006} &  \makecell{0.780\\±0.006} \\
\textbf{6     } &  \makecell{0.493\\±0.003} &  \makecell{0.223\\±0.013} &  \makecell{0.778\\±0.004} \\
\textbf{10    } &  \makecell{0.491\\±0.001} &  \makecell{0.208\\±0.019} &  \makecell{0.777\\±0.005} \\
\textbf{15    } &  \makecell{0.489\\±0.003} &  \makecell{0.181\\±0.011} &  \makecell{0.781\\±0.005} \\
\bottomrule
\end{tabular}


==> tables/daily_mc1024.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{9}{|c}{1024} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{1} & \multicolumn{3}{|c}{2} & \multicolumn{3}{|c}{4} \\
{} &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC \\
\textbf{Epochs} &                           &                           &                           &                           &                           &                           &                           &                           &                           \\
\midrule
\textbf{3     } &  \makecell{0.498\\±0.004} &  \makecell{0.176\\±0.013} &  \makecell{0.775\\±0.005} &  \makecell{0.494\\±0.003} &  \makecell{0.183\\±0.009} &  \makecell{0.778\\±0.006} &  \makecell{0.492\\±0.001} &  \makecell{0.194\\±0.010} &  \makecell{0.780\\±0.007} \\
\textbf{6     } &  \makecell{0.492\\±0.004} &  \makecell{0.162\\±0.015} &  \makecell{0.766\\±0.002} &  \makecell{0.488\\±0.001} &  \makecell{0.187\\±0.012} &  \makecell{0.774\\±0.003} &  \makecell{0.490\\±0.001} &  \makecell{0.198\\±0.015} &  \makecell{0.770\\±0.003} \\
\textbf{10    } &  \makecell{0.490\\±0.000} &  \makecell{0.168\\±0.012} &  \makecell{0.769\\±0.005} &  \makecell{\textbf{0.487}\\±0.002} &  \makecell{0.172\\±0.009} &  \makecell{0.770\\±0.003} &  \makecell{0.489\\±0.001} &  \makecell{0.193\\±0.006} &  \makecell{0.769\\±0.002} \\
\textbf{15    } &  \makecell{0.489\\±0.002} &  \makecell{0.161\\±0.009} &  \makecell{0.772\\±0.005} &  \makecell{0.488\\±0.004} &  \makecell{0.163\\±0.021} &  \makecell{0.772\\±0.004} &  \makecell{0.489\\±0.003} &  \makecell{0.172\\±0.023} &  \makecell{0.772\\±0.003} \\
\bottomrule
\end{tabular}


==> tables/daily_mc128.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{9}{|c}{128} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{64} & \multicolumn{3}{|c}{128} & \multicolumn{3}{|c}{256} \\
{} &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC \\
\textbf{Epochs} &                           &                           &                           &                           &                           &                           &                           &                           &                           \\
\midrule
\textbf{3     } &  \makecell{0.517\\±0.003} &  \makecell{0.205\\±0.004} &  \makecell{0.753\\±0.006} &  \makecell{0.519\\±0.004} &  \makecell{0.207\\±0.006} &  \makecell{0.763\\±0.003} &  \makecell{0.520\\±0.007} &  \makecell{0.210\\±0.005} &  \makecell{0.759\\±0.017} \\
\textbf{6     } &  \makecell{0.516\\±0.004} &  \makecell{0.223\\±0.006} &  \makecell{0.759\\±0.004} &  \makecell{0.526\\±0.001} &  \makecell{0.225\\±0.007} &  \makecell{0.754\\±0.001} &  \makecell{0.526\\±0.005} &  \makecell{0.230\\±0.008} &  \makecell{0.756\\±0.002} \\
\textbf{10    } &  \makecell{0.523\\±0.001} &  \makecell{0.229\\±0.005} &  \makecell{0.756\\±0.014} &  \makecell{0.529\\±0.005} &  \makecell{\textbf{0.232}\\±0.003} &  \makecell{0.756\\±0.016} &  \makecell{0.537\\±0.006} &  \makecell{0.227\\±0.004} &  \makecell{0.743\\±0.005} \\
\textbf{15    } &  \makecell{0.532\\±0.002} &  \makecell{0.227\\±0.006} &  \makecell{0.757\\±0.016} &  \makecell{0.541\\±0.008} &  \makecell{0.221\\±0.003} &  \makecell{0.751\\±0.017} &  \makecell{0.544\\±0.007} &  \makecell{0.222\\±0.002} &  \makecell{0.745\\±0.016} \\
\bottomrule
\end{tabular}


==> tables/daily_mc256.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{9}{|c}{256} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{16} & \multicolumn{3}{|c}{32} & \multicolumn{3}{|c}{64} \\
{} &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC \\
\textbf{Epochs} &                           &                           &                           &                           &                           &                           &                           &                           &                           \\
\midrule
\textbf{3     } &  \makecell{0.499\\±0.003} &  \makecell{0.207\\±0.001} &  \makecell{0.776\\±0.005} &  \makecell{0.500\\±0.005} &  \makecell{0.205\\±0.007} &  \makecell{0.777\\±0.009} &  \makecell{0.501\\±0.003} &  \makecell{0.207\\±0.005} &  \makecell{0.775\\±0.002} \\
\textbf{6     } &  \makecell{0.499\\±0.002} &  \makecell{0.214\\±0.006} &  \makecell{0.768\\±0.005} &  \makecell{0.498\\±0.003} &  \makecell{0.223\\±0.007} &  \makecell{0.769\\±0.001} &  \makecell{0.502\\±0.003} &  \makecell{0.228\\±0.007} &  \makecell{0.763\\±0.004} \\
\textbf{10    } &  \makecell{0.501\\±0.003} &  \makecell{0.223\\±0.010} &  \makecell{0.769\\±0.005} &  \makecell{0.507\\±0.001} &  \makecell{0.224\\±0.003} &  \makecell{0.771\\±0.004} &  \makecell{0.506\\±0.003} &  \makecell{0.227\\±0.016} &  \makecell{0.769\\±0.003} \\
\textbf{15    } &  \makecell{0.504\\±0.006} &  \makecell{0.211\\±0.011} &  \makecell{0.775\\±0.003} &  \makecell{0.511\\±0.004} &  \makecell{0.211\\±0.007} &  \makecell{0.775\\±0.005} &  \makecell{0.512\\±0.002} &  \makecell{0.208\\±0.012} &  \makecell{0.777\\±0.003} \\
\bottomrule
\end{tabular}


==> tables/daily_mc512.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{9}{|c}{512} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{4} & \multicolumn{3}{|c}{8} & \multicolumn{3}{|c}{16} \\
{} &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC \\
\textbf{Epochs} &                           &                           &                           &                           &                           &                           &                           &                           &                           \\
\midrule
\textbf{3     } &  \makecell{0.496\\±0.001} &  \makecell{0.193\\±0.008} &  \makecell{0.783\\±0.005} &  \makecell{0.492\\±0.002} &  \makecell{0.198\\±0.012} &  \makecell{\textbf{0.784}\\±0.007} &  \makecell{0.490\\±0.003} &  \makecell{0.202\\±0.004} &  \makecell{0.780\\±0.004} \\
\textbf{6     } &  \makecell{0.492\\±0.003} &  \makecell{0.195\\±0.007} &  \makecell{0.769\\±0.005} &  \makecell{0.494\\±0.002} &  \makecell{0.211\\±0.013} &  \makecell{0.768\\±0.005} &  \makecell{0.494\\±0.004} &  \makecell{0.218\\±0.008} &  \makecell{0.776\\±0.003} \\
\textbf{10    } &  \makecell{0.492\\±0.002} &  \makecell{0.201\\±0.012} &  \makecell{0.772\\±0.006} &  \makecell{0.490\\±0.003} &  \makecell{0.209\\±0.007} &  \makecell{0.770\\±0.007} &  \makecell{0.490\\±0.001} &  \makecell{0.214\\±0.012} &  \makecell{0.774\\±0.006} \\
\textbf{15    } &  \makecell{0.493\\±0.003} &  \makecell{0.186\\±0.007} &  \makecell{0.772\\±0.009} &  \makecell{0.493\\±0.002} &  \makecell{0.197\\±0.007} &  \makecell{0.775\\±0.004} &  \makecell{0.498\\±0.005} &  \makecell{0.197\\±0.009} &  \makecell{0.778\\±0.007} \\
\bottomrule
\end{tabular}


==> tables/daily_mc64.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{9}{|c}{64} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{256} & \multicolumn{3}{|c}{512} & \multicolumn{3}{|c}{1024} \\
{} &  MSAE &   IoU &   DPC &  MSAE &   IoU &   DPC &  MSAE &   IoU &   DPC \\
\textbf{Epochs} &       &       &       &       &       &       &       &       &       \\
\midrule
\textbf{3     } & 0.559 & 0.187 & 0.730 & 0.553 & 0.188 & 0.724 & 0.555 & 0.192 & 0.723 \\
\textbf{6     } & 0.565 & 0.199 & 0.730 & 0.565 & 0.199 & 0.731 & 0.571 & 0.194 & 0.720 \\
\textbf{10    } & 0.560 & 0.210 & 0.731 & 0.566 & 0.208 & 0.726 & 0.574 & 0.207 & 0.719 \\
\textbf{15    } & 0.569 & 0.209 & 0.729 & 0.579 & 0.205 & 0.722 & 0.584 & 0.204 & 0.714 \\
\bottomrule
\end{tabular}


==> tables/weekly_mc0.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{3}{|c}{0} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{0} \\
{} &                      MSAE &                       IoU &                       DPC \\
\textbf{Epochs} &                           &                           &                           \\
\midrule
\textbf{3     } &  \makecell{0.545\\±0.010} &  \makecell{0.156\\±0.008} &  \makecell{0.656\\±0.075} \\
\textbf{6     } &  \makecell{0.510\\±0.004} &  \makecell{0.188\\±0.006} &  \makecell{0.757\\±0.005} \\
\textbf{10    } &  \makecell{0.502\\±0.002} &  \makecell{0.204\\±0.007} &  \makecell{0.766\\±0.008} \\
\textbf{15    } &  \makecell{0.497\\±0.001} &  \makecell{0.208\\±0.005} &  \makecell{0.757\\±0.013} \\
\textbf{25    } &  \makecell{0.493\\±0.003} &  \makecell{0.205\\±0.009} &  \makecell{0.763\\±0.005} \\
\textbf{40    } &  \makecell{0.495\\±0.003} &  \makecell{0.192\\±0.011} &  \makecell{0.761\\±0.008} \\
\bottomrule
\end{tabular}


==> tables/weekly_mc1024.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{9}{|c}{1024} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{1} & \multicolumn{3}{|c}{2} & \multicolumn{3}{|c}{4} \\
{} &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC \\
\textbf{Epochs} &                           &                           &                           &                           &                           &                           &                           &                           &                           \\
\midrule
\textbf{3     } &  \makecell{0.554\\±0.003} &  \makecell{0.148\\±0.000} &  \makecell{0.671\\±0.039} &  \makecell{0.552\\±0.011} &  \makecell{0.151\\±0.011} &  \makecell{0.678\\±0.050} &  \makecell{0.545\\±0.003} &  \makecell{0.153\\±0.010} &  \makecell{0.710\\±0.022} \\
\textbf{6     } &  \makecell{0.511\\±0.003} &  \makecell{0.171\\±0.003} &  \makecell{0.754\\±0.012} &  \makecell{0.508\\±0.004} &  \makecell{0.185\\±0.001} &  \makecell{0.765\\±0.007} &  \makecell{0.508\\±0.002} &  \makecell{0.182\\±0.009} &  \makecell{0.766\\±0.007} \\
\textbf{10    } &  \makecell{0.503\\±0.005} &  \makecell{0.173\\±0.008} &  \makecell{0.761\\±0.013} &  \makecell{0.499\\±0.002} &  \makecell{0.180\\±0.012} &  \makecell{0.772\\±0.001} &  \makecell{0.497\\±0.002} &  \makecell{0.197\\±0.002} &  \makecell{0.771\\±0.006} \\
\textbf{15    } &  \makecell{0.498\\±0.002} &  \makecell{0.186\\±0.008} &  \makecell{0.762\\±0.011} &  \makecell{0.496\\±0.002} &  \makecell{0.193\\±0.008} &  \makecell{0.761\\±0.010} &  \makecell{0.493\\±0.002} &  \makecell{0.194\\±0.005} &  \makecell{0.772\\±0.009} \\
\textbf{25    } &  \makecell{0.493\\±0.004} &  \makecell{0.177\\±0.009} &  \makecell{0.751\\±0.006} &  \makecell{\textbf{0.489}\\±0.002} &  \makecell{0.186\\±0.012} &  \makecell{0.753\\±0.009} &  \makecell{\textbf{0.489}\\±0.001} &  \makecell{0.199\\±0.010} &  \makecell{0.758\\±0.005} \\
\textbf{40    } &  \makecell{0.493\\±0.002} &  \makecell{0.166\\±0.010} &  \makecell{0.752\\±0.013} &  \makecell{0.490\\±0.001} &  \makecell{0.178\\±0.009} &  \makecell{0.759\\±0.009} &  \makecell{\textbf{0.489}\\±0.002} &  \makecell{0.188\\±0.010} &  \makecell{0.762\\±0.014} \\
\bottomrule
\end{tabular}


==> tables/weekly_mc128.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{9}{|c}{128} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{64} & \multicolumn{3}{|c}{128} & \multicolumn{3}{|c}{256} \\
{} &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC \\
\textbf{Epochs} &                           &                           &                           &                           &                           &                           &                           &                           &                           \\
\midrule
\textbf{3     } &  \makecell{0.577\\±0.007} &  \makecell{0.145\\±0.005} &  \makecell{0.648\\±0.020} &  \makecell{0.582\\±0.004} &  \makecell{0.150\\±0.004} &  \makecell{0.653\\±0.024} &  \makecell{0.579\\±0.007} &  \makecell{0.139\\±0.017} &  \makecell{0.610\\±0.060} \\
\textbf{6     } &  \makecell{0.540\\±0.006} &  \makecell{0.186\\±0.012} &  \makecell{0.728\\±0.006} &  \makecell{0.539\\±0.003} &  \makecell{0.197\\±0.001} &  \makecell{0.742\\±0.010} &  \makecell{0.536\\±0.003} &  \makecell{0.194\\±0.006} &  \makecell{0.727\\±0.022} \\
\textbf{10    } &  \makecell{0.529\\±0.005} &  \makecell{0.205\\±0.002} &  \makecell{0.738\\±0.009} &  \makecell{0.532\\±0.007} &  \makecell{0.206\\±0.005} &  \makecell{0.754\\±0.004} &  \makecell{0.531\\±0.013} &  \makecell{0.207\\±0.000} &  \makecell{0.739\\±0.018} \\
\textbf{15    } &  \makecell{0.518\\±0.004} &  \makecell{0.208\\±0.003} &  \makecell{0.742\\±0.018} &  \makecell{0.518\\±0.005} &  \makecell{0.209\\±0.004} &  \makecell{0.753\\±0.013} &  \makecell{0.523\\±0.002} &  \makecell{0.215\\±0.001} &  \makecell{0.745\\±0.023} \\
\textbf{25    } &  \makecell{0.517\\±0.004} &  \makecell{0.212\\±0.006} &  \makecell{0.742\\±0.017} &  \makecell{0.517\\±0.002} &  \makecell{\textbf{0.220}\\±0.003} &  \makecell{0.752\\±0.002} &  \makecell{0.523\\±0.002} &  \makecell{0.217\\±0.004} &  \makecell{0.742\\±0.004} \\
\textbf{40    } &  \makecell{0.523\\±0.004} &  \makecell{0.219\\±0.002} &  \makecell{0.746\\±0.007} &  \makecell{0.527\\±0.003} &  \makecell{0.212\\±0.006} &  \makecell{0.746\\±0.003} &  \makecell{0.529\\±0.005} &  \makecell{0.216\\±0.001} &  \makecell{0.739\\±0.012} \\
\bottomrule
\end{tabular}


==> tables/weekly_mc256.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{9}{|c}{256} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{16} & \multicolumn{3}{|c}{32} & \multicolumn{3}{|c}{64} \\
{} &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC \\
\textbf{Epochs} &                           &                           &                           &                           &                           &                           &                           &                           &                           \\
\midrule
\textbf{3     } &  \makecell{0.555\\±0.003} &  \makecell{0.147\\±0.014} &  \makecell{0.682\\±0.028} &  \makecell{0.557\\±0.002} &  \makecell{0.155\\±0.005} &  \makecell{0.651\\±0.042} &  \makecell{0.560\\±0.001} &  \makecell{0.153\\±0.011} &  \makecell{0.656\\±0.045} \\
\textbf{6     } &  \makecell{0.516\\±0.003} &  \makecell{0.193\\±0.004} &  \makecell{0.753\\±0.005} &  \makecell{0.513\\±0.002} &  \makecell{0.199\\±0.005} &  \makecell{0.755\\±0.013} &  \makecell{0.513\\±0.001} &  \makecell{0.196\\±0.004} &  \makecell{0.751\\±0.011} \\
\textbf{10    } &  \makecell{0.507\\±0.003} &  \makecell{0.200\\±0.006} &  \makecell{0.755\\±0.013} &  \makecell{0.504\\±0.003} &  \makecell{0.206\\±0.007} &  \makecell{0.764\\±0.012} &  \makecell{0.506\\±0.002} &  \makecell{0.205\\±0.005} &  \makecell{0.761\\±0.009} \\
\textbf{15    } &  \makecell{0.502\\±0.004} &  \makecell{0.207\\±0.005} &  \makecell{0.766\\±0.003} &  \makecell{0.505\\±0.003} &  \makecell{0.210\\±0.005} &  \makecell{0.762\\±0.008} &  \makecell{0.501\\±0.002} &  \makecell{0.213\\±0.002} &  \makecell{0.758\\±0.004} \\
\textbf{25    } &  \makecell{0.499\\±0.003} &  \makecell{0.208\\±0.005} &  \makecell{0.762\\±0.007} &  \makecell{0.503\\±0.006} &  \makecell{0.214\\±0.005} &  \makecell{0.759\\±0.002} &  \makecell{0.500\\±0.006} &  \makecell{0.216\\±0.005} &  \makecell{0.763\\±0.005} \\
\textbf{40    } &  \makecell{0.500\\±0.001} &  \makecell{0.211\\±0.003} &  \makecell{0.762\\±0.003} &  \makecell{0.503\\±0.001} &  \makecell{0.212\\±0.009} &  \makecell{0.762\\±0.007} &  \makecell{0.507\\±0.004} &  \makecell{0.217\\±0.007} &  \makecell{0.758\\±0.003} \\
\bottomrule
\end{tabular}


==> tables/weekly_mc512.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{9}{|c}{512} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{4} & \multicolumn{3}{|c}{8} & \multicolumn{3}{|c}{16} \\
{} &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC &                      MSAE &                       IoU &                       DPC \\
\textbf{Epochs} &                           &                           &                           &                           &                           &                           &                           &                           &                           \\
\midrule
\textbf{3     } &  \makecell{0.554\\±0.005} &  \makecell{0.154\\±0.004} &  \makecell{0.702\\±0.023} &  \makecell{0.551\\±0.004} &  \makecell{0.157\\±0.008} &  \makecell{0.682\\±0.023} &  \makecell{0.551\\±0.004} &  \makecell{0.159\\±0.005} &  \makecell{0.668\\±0.028} \\
\textbf{6     } &  \makecell{0.512\\±0.004} &  \makecell{0.189\\±0.007} &  \makecell{0.760\\±0.015} &  \makecell{0.509\\±0.003} &  \makecell{0.191\\±0.005} &  \makecell{0.764\\±0.007} &  \makecell{0.509\\±0.001} &  \makecell{0.193\\±0.003} &  \makecell{0.764\\±0.009} \\
\textbf{10    } &  \makecell{0.501\\±0.003} &  \makecell{0.193\\±0.010} &  \makecell{0.771\\±0.003} &  \makecell{0.496\\±0.001} &  \makecell{0.198\\±0.010} &  \makecell{\textbf{0.777}\\±0.008} &  \makecell{0.500\\±0.004} &  \makecell{0.202\\±0.004} &  \makecell{0.772\\±0.007} \\
\textbf{15    } &  \makecell{0.498\\±0.001} &  \makecell{0.193\\±0.011} &  \makecell{0.764\\±0.011} &  \makecell{0.496\\±0.000} &  \makecell{0.205\\±0.006} &  \makecell{0.766\\±0.006} &  \makecell{0.496\\±0.001} &  \makecell{0.204\\±0.005} &  \makecell{0.772\\±0.008} \\
\textbf{25    } &  \makecell{0.495\\±0.001} &  \makecell{0.201\\±0.001} &  \makecell{0.766\\±0.004} &  \makecell{0.494\\±0.001} &  \makecell{0.205\\±0.008} &  \makecell{0.758\\±0.007} &  \makecell{0.495\\±0.002} &  \makecell{0.209\\±0.003} &  \makecell{0.760\\±0.007} \\
\textbf{40    } &  \makecell{0.494\\±0.003} &  \makecell{0.194\\±0.005} &  \makecell{0.761\\±0.003} &  \makecell{0.492\\±0.003} &  \makecell{0.200\\±0.007} &  \makecell{0.764\\±0.007} &  \makecell{0.491\\±0.002} &  \makecell{0.205\\±0.008} &  \makecell{0.766\\±0.005} \\
\bottomrule
\end{tabular}


==> tables/weekly_mc64.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Patch Size} & \multicolumn{9}{|c}{64} \\
\textbf{\#Patches} & \multicolumn{3}{|c}{256} & \multicolumn{3}{|c}{512} & \multicolumn{3}{|c}{1024} \\
{} &  MSAE &   IoU &   DPC &  MSAE &   IoU &   DPC &  MSAE &   IoU &   DPC \\
\textbf{Epochs} &       &       &       &       &       &       &       &       &       \\
\midrule
\textbf{3     } & 0.624 & 0.114 & 0.545 & 0.626 & 0.123 & 0.576 & 0.621 & 0.121 & 0.567 \\
\textbf{6     } & 0.587 & 0.178 & 0.678 & 0.585 & 0.176 & 0.713 & 0.581 & 0.185 & 0.711 \\
\textbf{10    } & 0.570 & 0.190 & 0.719 & 0.569 & 0.193 & 0.709 & 0.564 & 0.186 & 0.716 \\
\textbf{15    } & 0.561 & 0.193 & 0.722 & 0.559 & 0.191 & 0.715 & 0.563 & 0.193 & 0.723 \\
\bottomrule
\end{tabular}

